EquiHGNN: Scalable Rotationally Equivariant Hypergraph Neural Networks

Molecular interactions often involve high-order relationships that cannot be fully captured by traditional graph-based models limited to pairwise connections. Hypergraphs naturally extend graphs by enabling multi-way interactions, making them well-suited for modeling complex molecular systems. In this work, we introduce EquiHGNN, an Equivariant HyperGraph Neural Network framework that integrates symmetry-aware representations to improve molecular modeling. By enforcing the equivariance under relevant transformation groups, our approach preserves geometric and topological properties, leading to more robust and physically meaningful representations. We examine a range of equivariant architectures and demonstrate that integrating symmetry constraints leads to notable performance gains on large-scale molecular datasets. Experiments on both small and large molecules show that high-order interactions offer limited benefits for small molecules but consistently outperform 2D graphs on larger ones. Adding geometric features to these high-order structures further improves the performance, emphasizing the value of spatial information in molecular learning. Our source code is available at https://github.com/HySonLab/EquiHGNN/

==> tex/background.tex <==
\subsection{Message Passing}

Message Passing Neural Networks (MPNNs) play a fundamental role in learning node representations by propagating information along graph edges. As inherently permutation-invariant architectures, MPNNs effectively capture relational structures in graph-structured data, making them particularly well-suited for applications such as molecular modeling ~\cite{gilmer2017neural}.

Given a graph \(\mathcal{G} = (\mathcal{V}, \mathcal{E})\) with nodes \(v_i \in \mathcal{V}\) and edges \(e_{ij} \in \mathcal{E}\), each node \(v_i\) is associated with a feature vector \(\mathbf{h}_i \in \mathbb{R}^{c_n}\) and each edge \(e_{ij}\) with a feature vector \(\mathbf{a}_{ij} \in \mathbb{R}^{c_e}\), where \(c_n\) and \(c_e\) represent the dimensionalities of the node and edge features, respectively. The nodes representation are iteratively updated by:
\begin{equation}
\begin{aligned}
    \mathbf{m}_{ij} &= \phi_{e}(\mathbf{h}^l_i, \mathbf{h}^l_j, \mathbf{a}_{ij}) \\ 
    \mathbf{m}_i &= \text{AGGREGATE} \bigg( \{{\mathbf{m}_{ij}\}}_{j\in\mathcal{N}(i)} \bigg) \\
    \mathbf{h}^{l+1}_i &= \phi_{u}(\mathbf{h}^l_i, \mathbf{m}_i)
\end{aligned}
\end{equation}
where \(\mathcal{N}(i)\) denotes the set of neighbors of node \(v_i\), and the AGGREGATE function is a permutation-invariant operation over the neighbors (e.g., summation). The functions \(\phi_m\) and \(\phi_e\) are the message computation and feature update function, respectively, typically parameterized by multilayer perceptrons (MLPs). To obtain the final graph representation, a permutation-invariant aggregator is applied to the final hidden states of all nodes. However, this operation itself does not inherently preserve E(3) equivariance.

\subsection{Equivariance}

Equivariance is a property of functions that ensures information is preserved under transformations from a group \( G \). A function \( \phi: \mathcal{X} \to \mathcal{Y} \) is equivariant with respect to \( G \) if for all \( g \in G \) and \( x \in \mathcal{X} \), the following holds:
\[
\phi(g \cdot x) = g \cdot \phi(x).
\]
This property ensures that the output transforms in the same way as the input under transformations like rotation, translation, or scaling. In molecular modeling, equivariance to these symmetries (e.g., the rotation group \( SO(3) \)) is crucial because molecules retain their physical properties regardless of their orientation or position. 

% Should talk about Invariance / Equivariant

% MPNNs are designed to operate on discrete, unordered node sets, and do not inherently account for geometric symmetries. Without equivariance, these models lose important spatial information, leading to inaccurate predictions. Incorporating equivariance into GNNs ensures that the model respects these symmetries, preserving geometric consistency and leading to more robust and physically meaningful representations for tasks like molecular interaction prediction.

\subsection{Hypergraph}

A \textit{hypergraph} is a generalization of a graph where an edge, called a \textit{hyperedge}, can connect any number of nodes. Formally, a hypergraph is defined as: 
\[
\mathcal{H} = (\mathcal{V}, \mathcal{E}),
\] 
where \(\mathcal{V}\) is the set of nodes and \(\mathcal{E} \subseteq 2^{\mathcal{V}} \setminus \{\emptyset\}\) is the set of hyperedges, each representing a subset of nodes. Unlike traditional graphs that capture pairwise relationships, hypergraphs model higher-order interactions, making them ideal for complex systems such as protein interactions
~\cite{murgas2022hypergraph} and chemical reactions~\cite{schwaller2020predicting}.  

Hypergraph-based models extend GNNs to process hyperedges, allowing better representation of structured data. In molecular chemistry, hypergraphs effectively model \textit{conjugated structures}, where delocalized electrons form multi-atomic interactions crucial for optoelectronic properties. Recent studies demonstrate that HGNNs outperform traditional GNNs and 3D-based models in predicting molecular properties, offering a powerful approach for data-scarce applications like organic semiconductor design.

\subsection{Model details}
\label{model_overview}

\cref{tab:model_overview} outlines the architectural configurations of the models used in our experiments, including the number of parameters, layers, attention heads, and hidden dimensions.

\begin{table}[h]
    \centering
    \caption{Model Architecture Overview}
    \renewcommand{\arraystretch}{1.2}
    \label{tab:model_overview}
    \resizebox{\textwidth}{!}
    {
        \begin{tabular}{lcccc}
            \toprule[1pt]\midrule[0.3pt]
            Model & No.parameters & No.layers & No. attention heads & Hidden dimension\\
            \midrule
            GIN & 965K & 2 & - & 256 \\
            GAT & 3.7M & 2 & 4 & 256 \\
            % GATv2 & 5.5M \\        
            MHNN & 2.5M & 2 & - & 256 \\
            EGNN & 844K & 2 & 8 & 256 \\
            FAFormer & 3.2M & 2 & 2 & 256 \\
            Equiformer & 13M & 1 & 1 & 256 \\
            \midrule[0.3pt]\bottomrule[1pt]
        \end{tabular}
    }
\end{table}

